Trust, but Verify: Two-Phase Typing for Dynamic Languages

A key challenge when statically typing so-called dynamic languages is the ubiquity of value-based overloading, where a given function can dynamically reflect upon and behave according to the types of its arguments. Thus, to establish basic types, the analysis must reason precisely about values, but in the presence of higher-order functions and polymorphism, this reasoning itself can require basic types. In this paper we address this chicken-and-egg problem by introducing the framework of two-phased typing. The first "trust" phase performs classical, i.e. flow-, path- and value-insensitive type checking to assign basic types to various program expressions. When the check inevitably runs into "errors" due to value-insensitivity, it wraps problematic expressions with DEAD-casts, which explicate the trust obligations that must be discharged by the second phase. The second phase uses refinement typing, a flow- and path-sensitive analysis, that decorates the first phase's types with logical predicates to track value relationships and thereby verify the casts and establish other correctness properties for dynamically typed languages.

==> aux-first-phase.tex <==

\begin{figure*}[htpb]
% \begin{subfigure}[b]{0.5\textwidth}
\[
\begin{array}{ll}
  \typetag{\tnumber}                    & = \{\texttt{"number"}\}   \\
  \typetag{\tbool}                      & = \{\texttt{"boolean"}\}  \\
  % \typetag{\tvar}                       & = \text{\todo{???}} \\
  \typetag{\tfun{\type}{\type'}}       & = \{\texttt{"function"}\}  \\
  \typetag{\tand{\type}{\type'}}       & = \typetag{\type}          \\ 
  \typetag{\tor{\type}{\type'}}         & = \typetag{\type} \cup \typetag{\type'}
\end{array}
\]
% \end{subfigure}
% \begin{subfigure}[b]{0.5\textwidth}
% \[
% \begin{array}{ll}
%   \nointer{\tprim}                       & = \vtrue  \\
%   \nointer{\tfun{\type}{\type'}}        & = \nointer{\type} \wedge \nointer{\type'} \\
%   \nointer{\tand{\type}{\type'}}        & = \vfalse          \\ 
%   \nointer{\tor{\type}{\type'}}         & =  \nointer{\type} \wedge \nointer{\type'}
% \end{array}
% \]
% \end{subfigure}
\caption{Auxiliary definitions for First Phase}
\label{fig:firstphaseaux}
\end{figure*}

% 
% \begin{figure*}[htpb]
% \begin{subfigure}[b]{0.5\textwidth}
% \[
% \begin{array}{ll}
%   \typetag{\tnumber}                    & = \{\texttt{"number"}\}   \\
%   \typetag{\tbool}                      & = \{\texttt{"boolean"}\}  \\
%   % \typetag{\tvar}                       & = \text{\todo{???}} \\
%   \typetag{\tfun{\type}{\type'}}       & = \{\texttt{"function"}\}  \\
%   \typetag{\tand{\type}{\type'}}       & = \typetag{\type}          \\ 
%   \typetag{\tor{\type}{\type}}         & = \typetag{\type} \cup \typetag{\type} \\  \\  [0.12in]
% \end{array}
% \]
% \end{subfigure}
% \begin{subfigure}[b]{0.5\textwidth}
% \[
% \begin{array}{ll}
% \match{\type}{\type'}                                 & = \issubtype{\type}{\type'} \vee \issubtype{\type'}{\type}  \\
%         [0.12in]
%   \tjoin{\type_1}{\type_2}
%    & =
%     \begin{cases}
%       \type_1 & \text{if } \issubtype{\type_2}{\type_1}  \\
%       \type_2 &  \text{if } \issubtype{\type_1}{\type_2}  \\
%       \die    &  \text{otherwise}
%     \end{cases} \\   [0.30in]
% \end{array}
% \]
% \end{subfigure}
% \\
% \[
% \begin{array}{ll}
%   \resolveoverload 
%     {(\tfun{\tvar}{\type}{\type'}):{\many{\type}}}{\type} & =
%   \begin{cases}
%   \appsubst{\subst}{(\tfun{\type}{\type'})}
%     & \text{if } \existsi{\subst \equiv \tsubst{\tvar}{\type}}{\convert{\type}{\appsubst{\subst}{\type}}{\upcast{}{}}} \\
%   \resolveoverload {\many{\type}}{\type} & \text{otherwise}
%   \end{cases}   \\ [0.20in]
%   \resolveoverload{[\;]}{\twhatever} & = \tfun{\tbot}{\tbot}
% %
% %%
% %%
% %%
% %% \tjoin{\tprim}{\tprim}                   & = & \tprim    \\
% %% \tjoin{\tvar}{\tvar}                     & = & \tvar     \\
% %% \tjoin{\tfun{\many{\tbase_i}}{\tbase}}   
% %%       {\tfun{\many{\tbase_i'}}{\tbase'}} & = & \tfun{\many{\tjoin{\tbase_i}{\tbase_i'}}}{\tjoin{\tbase}{\tbase'}} \\
% %% \tjoin{\quant{\many{\tvar_i}} \tbase}
% %%       {\quant{\many{\tvar_i}} \tbase'}   & = & {\quant{\many{\tvar_i}} \tjoin{\tbase}{\tbase'}}   \\ 
% %% \tjoin{\tobj{\methts_1}{\fieldts_1}}
% %%       {\tobj{\methts_2}{\fieldts_2}}       
% %%   & = & \auxifthen{\existsi{\metht_1 \in \methts_1, \metht_2 \in \methts_2}
% %%     {\eqbind{$\metht_1$}{$\metht_2$} \imp \mtjoin{\metht_1}{\metht_2} = \die}}{\die} \\
% %%   &   & \auxletin{\methts}{\{  \mtjoin{\metht_1}{\metht_2}\ |\ \metht_1 \in \methts_1, \metht_2 \in \methts_2
% %%                     , \eqbind{$\metht_1$}{$\metht_2$} \}} \\
% %%   &   & \auxifthen{\existsi
% %%           {\fieldtdef{\type_1} \in \fieldts_1, \fieldtdef{\type_2} \in \fieldts_2}
% %%           {\tjoin{\type_1}{\type_2} = \die}
% %%         }{\die} \\
% %%   &   & \auxletin{\fieldts}{\{ \fieldtdef{\type}\ |\ \fieldtdef{\type_1} \in \fieldts_1
% %%                 ,\fieldtdef{\type_2} \in \fieldts_2, \type = \tjoin{\type_1}{\type_2} \}} \\
% %%   &   &  \tobj{\methts}{\fieldts} \\ [0.12in]
% %% \tjoin{\twhatever}{\twhatever}           & = & \die      \\ [0.12in]
% %% %
% %% \mtjoin{\methtdef{m}{\tvar}{\type_{\self,1}}{\type_{i,1}}{\type_1}}
% %%                  {\methtdef{n}{\tvar}{\type_{\self,2}}{\type_{i,2}}{\type_2}} 
% %%   & = & \auxifthen{m = n\ \wedge\ \many{\tjoin{\type_{i,1}}
% %%              {\type_{i,2}}} = \many{\type}\ \wedge\ \tjoin{\type_1}{\type_2} = \type''} \\
% %%   &   & \quad \auxreturn{\methtdef{m}{\tvar}{\type_{\self}}{\type}{\type}}  \\
% %%   &   & \die                                                                \\ [0.12in]
% %% %
% %% \resolveoverload{ {\left(  
% %%       \methtdef{m_{\overload}}{\tvar_i}{\type_{\self}}{\type_j}{\type}
% %%                    \right)} : {\methts}}{\many{\type_i}}{\many{\type_j}} 
% %%   & = & \auxifthen{\issubtype{\type_j}{\appsubst{\tsubsts{\tvar_i}{\type_i}}{\type_j}}} \\
% %%   &   & \quad\auxreturn{\methtdef{m_{\overload}}{\tvar_i}{\type_{\self}}{\type_j}{\type}}  \\
% %%   &   & \resolveoverload{\methts}{\many{\type_i}}{\many{\type_j}}   \\
% %% \resolveoverload{\twhatever}{\twhatever}{\twhatever} & = & \die \\
% %%
% \end{array}
% \]
% 
% \caption{Auxiliary definitions for First Phase}
% \label{fig:firstphaseaux}
% \end{figure*}
% 


==> cor-error-value.tex <==

\begin{corollary}[Error Value] \label{corollary:errorvalue} 
$\nexistsi{\texpr}{\steps{\deadcast{\type}{\unit}}{\texpr}}$
\end{corollary}


==> fig-elaboration-example.tex <==

\begin{figure}[!ht]
  \judgementHead{Example Typing Derivation}{\eletin{f}
       {\elambda
         {\evar}
         {\ite{\isnumber{\evar}}
              {\parens{\app{\minus}{\evar}}}
              {\parens{\app{\lnot}{\evar}}}}
          {}
       }
     {\app{f}{5}}}
\begin{mathpar}
\inferrule*[left=$\mathcal{D}_{12}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchkvar]
    {
    }
    {\translax{\tcenvext{\evar}{\tnm}}
              {\isnumber{\evar}}
              {\tbl}
              {\elabnointer}
              {\isnumber{\evar}}
    }$
}
}
\and
\inferrule*[left=$\mathcal{D}_{12}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchkapp]
    {
      \inferrule*[left=\tchkvar]
        {\envbinding{\evar}{\tfun{\tnm}{\tnm}} \in \tcenv}
        {\translax{\tcenvext{\evar}{\tnm}}
                {\parens{\minus}}
                {\tfun{\tnm}{\tnm}}
                {\elabnointer}
                {\parens{\minus}}
        }
      \\
      \inferrule*[left=\tchkvar]
        {
        }
        {\translax{\tcenvext{\evar}{\tnm}}
                {\evar}
                {\tnm}
                {\elabnointer}
                {\evar}
        }
    }
    {\translax{\tcenvext{\evar}{\tnm}}
              {\parens{\app{\minus}{\evar}}}
              {\tnm}
              {\elabnointer}
              {\parens{\app{\minus}{\evar}}}
    }$
}
}
\and
\inferrule*[left=$\mathcal{D}_{13}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchkapp]
  {
    \inferrule[]
    {}
    {
      \translax{\tcenvext{\evar}{\tnm}}
               {\parens{\lnot}}
               {\tfun{\tbl}{\tbl}}
               {\elabnointer}
               {\parens{\lnot}}
    }
    \\
    \inferrule*[left=\tchkdead]
    {
      \inferrule*[left=\tchkvar]
      {
      }
      {
        \translax{\tcenvext{\evar}{\tnm}}
                 {\evar}
                 {\tnm}
                 {\elabnointer}
                 {\evar}
      }
    }
    {
      \translax{\tcenvext{\evar}{\tnm}}
               {\evar}
               {\tbl}
               {\elabnointer}
               {\deadcast{\tbl}{\evar}}
    }
  }
  {\translax{\tcenvext{\evar}{\tnm}}
            {\parens{\app{\lnot}{\evar}}}
            {\tbl}
            {\elabnointer}
            {\app{\lnot}{\deadcast{\tbl}{\evar}}}
  }$
}
}
\and
%%%  D1
\inferrule*[left=$\mathcal{D}_{1}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchklambda]
  {
    \inferrule*[left=\tchkite]
    {
      \mathcal{D}_{11}
      \\
      \mathcal{D}_{12}
      \\
      \inferrule*[left=\tchkdead]
      {\mathcal{D}_{13}}
      {\translax{\tcenvext{\evar}{\tnm}}
                {\parens{\app{\lnot}{\evar}}}
                {\tnm}
                {\elabnointer}
                {\deadcast{\tnm}{\app{\lnot}{\evar}}}
      }
    }
    {\translax{\tcenvext{\evar}{\tnm}}
              {\ite{\isnumber{\evar}}
                   {\parens{\app{\minus}{\evar}}}
                   {\parens{\app{\lnot}{\evar}}}
              }
              {\tnm}
              {\elabnointer}
              {\ite{\isnumber{\evar}}
                   {\parens{\app{\minus}{\evar}}}
                   {\parens{\deadcast{\tnm}{\app{\lnot}{\evar}}}}
              }
    }
  }
  {\translax
    {\tcenv}
    {\underbrace{\elambda
      {\evar}
      {\ite{\isnumber{\evar}}
           {\parens{\app{\minus}{\evar}}}
           {\parens{\app{\lnot}{\evar}}}}
      {}
    }_{\texttt{neg}}}
    {\underbrace{\tfun{\tnm}{\tnm}}_{\II}}
    {\elabnointer}
    {\underbrace{\elambda
      {\evar}
      {\ite{\isnumber{\evar}}
           {\parens{\app{\minus}{\evar}}}
           {\parens{\deadcast{\tnm}{\app{\lnot}{\evar}}}}
         }
      {}
      }_{\texttt{neg}_1}}
}$
}
}
\and
%%%  D2
\inferrule*[left=$\mathcal{D}_{2}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchklambda]
  { 
    \vdots
  }
  {\translax
    {\tcenv}
    {\underbrace{\elambda
      {\evar}
      {\ite{\isnumber{\evar}}
           {\parens{\app{\minus}{\evar}}}
           {\parens{\app{\lnot}{\evar}}}}
      {}
    }_{\texttt{neg}}}
    {\underbrace{\tfun{\tbl}{\tbl}}_{\BB}}
    {\elabnointer}
    {\underbrace{\elambda
      {\evar}
      {\ite{\isnumber{\evar}}
        {\parens{\deadcast{\tbl}{\app{\minus}{\evar}}}}
           {\parens{\app{\lnot}{\evar}}}
      }
      {}
      }_{\texttt{neg}_2}}
}$
}
}
\and
%%%  D2
\inferrule*[left=$\mathcal{D}$]{}{
\colorbox{light-gray}{
  $\inferrule*[left=\tchkinterintro]
  {
    \mathcal{D}_1  \\   \mathcal{D}_2
  }
  {\translax
    {\tcenv}
    {\texttt{neg}}
    {\tand{\II}{\BB}}
    {\elabnointer}
    {\pair{\texttt{neg}_1}{\texttt{neg}_2}}
  }
$
}
}
\and
\inferrule*[left=\tchkletin]
{
  \mathcal{D}
  \\
  \inferrule*[left=\tchkapp]
  {
    \inferrule*[left=\tchkinterelim]
    {
      \translax{\tcenvext{f}{\tand{\II}{\BB}}}
               {f}
               {\tand{\II}{\BB}}
               {\elabnointer}
               {f}
    }
    {
      \translax{\tcenvext{f}{\tand{\II}{\BB}}}
               {f}
               {\II}
               {\elabinter}
               {\proj{1}{f}}
    }
    \and
    \inferrule[]
    {}
    {\transstrict{\emp}{5}{\tnm}{\elabnointer}{5}}
  }
  {
    \translax{\tcenvext{f}{\tand{\II}{\BB}}}
             {\app{f}{5}}
             {\tnm}
             {\elabnointer}
             {\app{(\proj{1}{f})}{5}}
  }
}
{
  \translax{\tcenv}
           {\eletin{f}{\texttt{neg}}{\app{f}{5}}}
           {\tnm}
           {\elabnointer}
           {\eletin{f}{\pair{\texttt{neg}_1}{\texttt{neg}_2}}{\app{(\proj{1}{f})}{5}}}
}
\end{mathpar}
\caption{Example Typing Derivation}
\label{fig:elaboration:example}
\end{figure}




==> lemma-no-dead-on-let-binding.tex <==

\begin{lemma}[No \tdead on let-binding] \label{lemma:no:dead:let}
%
If 
$$\trans{\tcenv}
       {\eletin{\evar}{\val_1}{\expr_2}}
       {\type}{}
       {\eletin{\evar}{\texpr_1}{\texpr_2}}$$
%
then there exists $\tval_1$ such that:
\begin{enumerate}[label={(\arabic*)}]
\inditem $\stepsmany{\texpr_1}{\tval_1}$
\inditem 
  $\trans{\tcenv}
         {\eletin{\evar}{\val_1}{\expr_2}}
         {\type}{}
         {\eletin{\evar}{\tval_1}{\texpr_2}}$
%
\end{enumerate}
\end{lemma}



==> lemma-no-dead-on-lhs-of-app.tex <==

\begin{lemma}[No \tdead on the left-hand side of application] \label{lemma:no:dead:lhsapp}
%
If 
$$\trans{\tcenv}
       {\app{\parens{\elambda{\evar}{\expr_0}{}}}{\expr_2}}
       {\tfun{\type}{\typeb}}{}
       {\app{\texpr_1}{\texpr_2}}$$
%
then there exists $\elambda{\evar}{\texpr_0}{}$ such that:
\begin{enumerate}[label={(\arabic*)}]
\inditem $\stepsmany{\texpr_1}{\elambda{\evar}{\texpr_0}{}}$
\inditem 
  $\trans{\tcenv}
       {\app{\parens{\elambda{\evar}{\expr_0}{}}}{\expr_2}}
         {\tfun{\type}{\typeb}}{}
         {\app{\parens{\elambda{\evar}{\texpr_0}{}}}{\texpr_2}}$
%
\end{enumerate}
\end{lemma}



==> lemma-type-preserve.tex <==

\begin{lemma}[Elaboration Type Soundness]\label{lemma:elabsound}
  If $\trans{\tcenv}{\expr}{\type}{}{\texpr}$ then 
$\infertarget{\elabtype{\tcenv}}{\texpr}{\elabtype{\type}}$.
\end{lemma}

\begin{proof}
\todo{Induction on the given derivation.}


\end{proof}


==> rules-source-subtyping.tex <==

\begin{figure}[ht]
\judgementHead{Subtyping}{\issubtype{\type}{\type'}}
%%                    {\issubtype{\metht_1}{\metht_2}}
%%                    {\issubtype{\fieldt_1}{\fieldt_2}}
\begin{mathpar}
  \inferrule
  [\subrefl]
  {}
  {\issubtype{\type}{\type}}
\and
\inferrule
  [\subunionleft]
  {\issubtype{\stype_i}{\type}}
  {\issubtype{\tor{\stype_1}{\stype_2}}{\type}}
\and
\inferrule
  [\subunionright]
  {\issubtype{\stype}{\type_1} \\ \issubtype{\stype}{\type_2}}
  {\issubtype{\stype}{\tor{\type_1}{\type_2}}}
\\
  \inferrule
  [\subinterleft]
  {\issubtype{\stype_1}{\type} \\ \issubtype{\stype_2}{\type}}
  {\issubtype{\tand{\stype_1}{\stype_2}}{\type}}
\and
  \inferrule
  [\subinterright]
  {\issubtype{\stype}{\type_i}}
  {\issubtype{\stype}{\tand{\type_1}{\type_2}}}
\and
  \inferrule
  [\subfun]
  {\foralli{i}{\issubtype{\type_i'}{\type_i}} \\ \issubtype{\type}{\type'}}
  {\issubtype{\tfun{\tvar}{\stype}{\type}}{\tfun{\tvar}{\stype'}}{\type'}}
%%%%
%%%% OBECTS AND CLASSES BELOW
%%%%
%%   \inferrule
%%   [\subobj]
%%   { \foralli {{\metht_2} \in {\many{\metht_2}}}{\exists {\metht_1} \in {\many{\metht_1}}\ \st\  
%%     \issubtype{\metht_1}{\metht_2}} \\\\
%%     \foralli {{\fieldt_2} \in {\many{\fieldt_2}}}{\exists {\fieldt_1} \in {\many{\fieldt_1}} \ \st\ 
%%     \issubtype{\fieldt_1}{\fieldt_2}}
%%   }
%%   {\issubtype{\tobj{\many{\metht_1}}{\many{\fieldt_1}}}{\tobj{\many{\metht_2}}{\many{\fieldt_2}}}}
%% \and
%%   \inferrule
%%   [\subtrefobj]
%%   {
%%     \tostruct{\tref{C}{\many{\type}}}{\tdefs} = {\tobj{\many{\metht}'}{\many{\fieldt}'}} \\\\
%%     \issubtype{\tobj{\many{\metht}'}{\many{\fieldt}'}}{\tobj{\many{\metht}}{\many{\fieldt}}}
%%   }
%%   {\issubtype{\tref{C}{\many{\type}}}{\tobj{\many{\metht}}{\many{\fieldt}}}}
%% \and
%%   \inferrule
%%   [\subtyprefa]
%%   {
%%     \weaken{\tdefs}{\tref{C_1}{\many{\type_1}}}{C_2} = \tref{C_2}{\many{\type_1}'} \\\\
%%     \issubtype{\tref{C_2}{\many{\type_1}'}}{\tref{C_2}{\many{\type_2}}}
%%   }
%%   {\issubtype{\tref{C_1}{\many{\type_1}}}{\tref{C_2}{\many{\type_2}}}}
%% \and
%%   \inferrule
%%   [\subtyprefb]
%%   {
%%     \tydefshort{C}{\many{\varp\;\tvar}} \in \tdefs \\\\
%%     \foralli{i}{\auxifthen{\varp_i \in \{+,\star\}}{\issubtype{\type_{1,i}}{\type_{2,i}}}} \\\\
%%     \foralli{i}{\auxifthen{\varp_i \in \{-,\star\}}{\issubtype{\type_{2,i}}{\type_{1,i}}}}
%%   }
%%   {\issubtype{\tref{C}{\many{\type_1}}}{\tref{C}{\many{\type_2}}}}
%% \\
%%   \inferrule
%%   [\submeth]
%%   {
%%     \issubtype{\type_{1,\self}}{\type_{2,\self}} \\ 
%%     \foralli{i} {\issubtype{\type_{2,i}}{\type_{1,i}}} \\ 
%%     \issubtype{\type_1'}{\type_2'}
%%   }
%%   {\issubtype{\methtdef{m_{\overload_1}}{\tvar}{\type_{1,\self}}{\type_1}{\type_1'}}
%%              {\methtdef{m_{\overload_2}}{\tvar}{\type_{2,\self}}{\type_2}{\type_2'}}
%%   }
%% \and
%%   \inferrule
%%   [\subfield]
%%   {\issubtype{\type_1}{\type_2}}
%%   {\issubtype{\fieldtdef{\type_1}}{\fieldtdef{\type_2}}}
\end{mathpar}
\vspace{\judgevspace}

\judgementHead{Type Conversion}{\convert{\type}{\type'}{\castd}}
\begin{mathpar}
\and
  \inferrule
  [\convupcast]
  {\issubtype{\stype}{\type}}
  {\convert{\stype}{\type}{\upcast{}{}}}
\and
  \inferrule
  [\convdowncast]
  {\stype_i = \type}
  {\convert{\tor{\stype_1}{\stype_2}}{\type}{\downcast{}{}}}
%%   \inferrule
%%   [\convdowncast]
%%   {C_1 \neq C_2 \\ \issubtype{C_2}{C_1}}
%%   {\convert{C_1}{C_2}{\downcast{}{}}}
%% %  
\and  
  \inferrule
  [\convdeadcast]
  {
    \nosubtype{\type}{\stype} \\ 
    \left(\stype \equiv \tor{\stype_1}{\stype_2}\right) \imp \foralli{i}{\nosubtype{\stype_i}{\type}}
  }
  {\convert{\stype}{\type}{\deadcast{}}}
\end{mathpar}
\caption{Subtyping Rules for Unrefined Types}
\label{fig:subtyping}
\end{figure}




==> rules-source-type-wf.tex <==
\begin{figure}[t!]
% \vspace{\judgevspace}
\judgementHead{Well-Formed Types}{\tcwf{\type}}
\begin{mathpar}
  \inferrule{}{\tcwf{\tprim}}
% \and
%   \inferrule{}{\tcwf{\tbot}}
\and
  \inferrule
  {
    \tcwf{\type}  \\ 
    \tcwf{\typeb} \\ 
    % \nointer{\tfun{\type}{\typeb}}  
  }
  {\tcwf{\tfun{\type}{\typeb}}}
\and
  \inferrule
  {\tcwf{\type} \\ \tcwf{\typeb} \\\\ \typetag{\type} = \typetag{\typeb}}
  {\tcwf{\tand{\type}{\typeb}}}
\and
  \inferrule
  {\tcwf{\type} \\ \tcwf{\typeb} \\\\ \typetag{\type}\cap \typetag{\typeb} = \emptyset}
  {\tcwf{\tor{\type}{\typeb}}}
%% \inferrule
%% {\foralli{i}{\tcwf{\type_i}}}
%% {\tcwf{\tref{C}{\many{\type_i}}}}
%% \and
%% \inferrule
%%   { \tcwf{\methts}\\
%%     \tcwf{\fieldts} }
%%   {\tcwf{\deftobj}}
%% \and
%% \inferrule 
%% {
%%   \foralli {\metht_1, \metht_2 \in \methts} 
%%            {\neg\issubtype{\metht_1}{\metht_2} \wedge  \neg\issubtype{\metht_2}{\metht_1}} \\
%%   %\forall \left(\methtdef{m_{\overload_1}}{\tvar}{\type_{\self,1}}{\type_{i,1}}{\type_1'}\right),
%%   %\left(\methtdef{m_{\overload_2}}{\tvar}{\type_{\self,2}}{\type_{i,2}}{\type_2'}\right)
%%   %       \in \methts\ . \ (\overload_1 \neq \overload_2) \imp 
%%   %     \neg{\left(\many{\issubtype{\type_{i,1}}{\type_{i,2}}} \wedge \issubtype{\type_2'}{\type_1'}\right)} \wedge
%%   %     \neg{\left(\many{\issubtype{\type_{i,2}}{\type_{i,1}}} \wedge \issubtype{\type_1'}{\type_2'}\right)} \\\\
%%   \foralli{\left(\methtdef{m_{\overload}}{\tvar}{\type_{\self}}{\type_i}{\typeb}\right) \in \methts}
%%   {\left\{\foralli{i}{\many{\tcwf{\type_i}}} \qquad \tcwf{\typeb}\right\}}
%% }
%% {\tcwf{\methts}}
%% \and 
%% \inferrule
%% {\foralli{\fieldtdef{\type} \in \fieldt}{\tcwf{\type}}}
%% {\tcwf{\fieldts}}
\end{mathpar}
\[
\begin{array}{lllll}
  \typetag{\tnumber}  & = \{\texttt{"number"}\}   & \qquad\qquad\qquad & \typetag{\tand{\type}{\type'}} & = \typetag{\type}          \\ 
  \typetag{\tbool}    & = \{\texttt{"boolean"}\}  &        & \typetag{\tor{\type}{\type'}}  & = \typetag{\type} \cup \typetag{\type'} \\
  \typetag{\tfun{\type}{\type'}}  & = \{\texttt{"function"}\}  & & & 
\end{array}
\]
\caption{Basic Type Well-Formedness} %  \bc{is Tag(unit) undefined?} PV: we rule out the unit type
\label{fig:source:wf}
\end{figure}




==> theorem-multi-consistency.tex <==

\begin{theorem}[Multi-step Consistency]\label{thr:multistep-consistency}
If $\transvar{\emp}{\expr}{\type}{}{\texpr}$ and $\stepsmany{\texpr}{}{\tval}$ then there
exists $\val$ such that $\stepsmany{\expr}{\val}$ and $\transvar{\emp}{\val}{\type}{}{\tval}$.
\end{theorem}

\begin{proof}
  Given by \cite{Dunfield2012} theorem 14.
\end{proof}



==> theorem-target-typesafe.tex <==

\begin{theorem}[Refinement Type Safety]\label{theorem:targettypesafe}
If $\infertarget{\emp}{\texpr}{\rtype}$ then either $\texpr$ is a value or
there exists $\texpr'$ such that $\steps{\texpr}{\texpr'}$ and
$\infertarget{\emp}{\texpr'}{\rtype}$.
\end{theorem}

\begin{proof}
  Given by Rondon \etal~\cite{LiquidPLDI08} for a similar language.
\end{proof}

